Statistical Patterns of Theory Uncertainties

A comprehensive uncertainty estimation is vital for the precision program of the LHC. While experimental uncertainties are often described by stochastic processes and well-defined nuisance parameters, theoretical uncertainties lack such a description. We study uncertainty estimates for cross-section predictions based on scale variations across a large set of processes. We find patterns similar to a stochastic origin, with accurate uncertainties for processes mediated by the strong force, but a systematic underestimate for electroweak processes. We propose an improved scheme, based on the scale variation of reference processes, which reduces outliers in the mapping from leading order to next-to-leading-order in perturbation theory.

==> pulls_ref.tex <==
\texttt{p p > wpm} 	 &1 & $1.54 \times 10^{-1}$ & 1.84 & \texttt{p p > t t~} 	 &2 & $1.45 \times 10^{-1}$ & 1.95 \\ 
\texttt{p p > wpm j} 	 &1 & $1.97 \times 10^{-1}$ & 1.96 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 1.33 \\ 
\texttt{p p > wpm j j } 	 &1 & $2.45 \times 10^{-1}$ & 0.59 & \texttt{p p > t t~ j } 	 &3 & $4.51 \times 10^{-1}$ & 0.32 \\ 
\texttt{p p > wpm j j j } 	 &1 & $4.10 \times 10^{-1}$ & 0.25 & \texttt{p p > t t~ j j } 	 &4 & $6.14 \times 10^{-1}$ & 0.17 \\ 
\texttt{p p > z} 	 &1 & $1.46 \times 10^{-1}$ & 1.87 & \texttt{p p > t t~} 	 &2 & $1.45 \times 10^{-1}$ & 1.88 \\ 
\texttt{p p > z j } 	 &1 & $1.93 \times 10^{-1}$ & 1.82 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 1.21 \\ 
\texttt{p p > z j j } 	 &1 & $2.43 \times 10^{-1}$ & 0.56 & \texttt{p p > t t~ j } 	 &3 & $4.51 \times 10^{-1}$ & 0.30 \\ 
\texttt{p p > z j j j } 	 &1 & $4.08 \times 10^{-1}$ & 0.27 & \texttt{p p > t t~ j j } 	 &4 & $6.14 \times 10^{-1}$ & 0.18 \\ 
\texttt{p p > a j } 	 &1 & $3.12 \times 10^{-1}$ & 5.33 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 5.74 \\ 
\texttt{p p > a j j } 	 &1 & $3.28 \times 10^{-1}$ & 0.85 & \texttt{p p > t t~ j } 	 &3 & $4.51 \times 10^{-1}$ & 0.62 \\ 
\texttt{p p > w+ w-} 	 &2 & $5.00 \times 10^{-2}$ & 7.99 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 1.38 \\ 
\texttt{p p > z z} 	 &2 & $4.50 \times 10^{-2}$ & 6.46 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 1.00 \\ 
\texttt{p p > z wpm} 	 &2 & $3.60 \times 10^{-2}$ & 17.09 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 2.12 \\ 
\texttt{p p > a a } 	 &2 & $2.21 \times 10^{-1}$ & 7.36 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 5.61 \\ 
\texttt{p p > a z } 	 &2 & $9.90 \times 10^{-2}$ & 4.73 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 1.61 \\ 
\texttt{p p > a wmp} 	 &2 & $9.50 \times 10^{-2}$ & 14.88 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 4.87 \\ 
\texttt{p p > w+ w- j } 	 &2 & $1.16 \times 10^{-1}$ & 2.58 & \texttt{p p > t t~ j } 	 &3 & $4.51 \times 10^{-1}$ & 0.66 \\ 
\texttt{pp > z z j } 	 &2 & $1.09 \times 10^{-1}$ & 2.93 & \texttt{p p > t t~ j } 	 &3 & $4.51 \times 10^{-1}$ & 0.71 \\ 
\texttt{p p > z wmp j } 	 &2 & $1.16 \times 10^{-1}$ & 2.57 & \texttt{p p > t t~ j } 	 &3 & $4.51 \times 10^{-1}$ & 0.66 \\ 
\texttt{p p > a a j } 	 &2 & $2.03 \times 10^{-1}$ & 6.13 & \texttt{p p > t t~ j } 	 &3 & $4.51 \times 10^{-1}$ & 2.76 \\ 
\texttt{p p > a z j } 	 &2 & $1.45 \times 10^{-1}$ & 3.23 & \texttt{p p > t t~ j } 	 &3 & $4.51 \times 10^{-1}$ & 1.04 \\ 
\texttt{p p > a wpm j } 	 &2 & $1.37 \times 10^{-1}$ & 3.32 & \texttt{p p > t t~ j } 	 &3 & $4.51 \times 10^{-1}$ & 1.01 \\ 
\texttt{p p > w+ w+ j j } 	 &2 & $2.54 \times 10^{-1}$ & 2.05 & \texttt{p p > t t~ j j } 	 &4 & $6.14 \times 10^{-1}$ & 0.85 \\ 
\texttt{p p > w- w- j j } 	 &2 & $2.54 \times 10^{-1}$ & 1.90 & \texttt{p p > t t~ j j } 	 &4 & $6.14 \times 10^{-1}$ & 0.78 \\ 
\texttt{p p > w+ w- j j } 	 &2 & $2.72 \times 10^{-1}$ & 0.84 & \texttt{p p > t t~ j j } 	 &4 & $6.14 \times 10^{-1}$ & 0.37 \\ 
\texttt{p p > z z j j } 	 &2 & $2.66 \times 10^{-1}$ & 1.04 & \texttt{p p > t t~ j j } 	 &4 & $6.14 \times 10^{-1}$ & 0.45 \\ 
\texttt{p p > z wpm j j} 	 &2 & $2.67 \times 10^{-1}$ & 0.51 & \texttt{p p > t t~ j j } 	 &4 & $6.14 \times 10^{-1}$ & 0.22 \\ 
\texttt{p p > a a j j } 	 &2 & $2.62 \times 10^{-1}$ & 1.50 & \texttt{p p > t t~ j j } 	 &4 & $6.14 \times 10^{-1}$ & 0.64 \\ 
\texttt{p p > a z j j } 	 &2 & $2.43 \times 10^{-1}$ & 1.24 & \texttt{p p > t t~ j j } 	 &4 & $6.14 \times 10^{-1}$ & 0.49 \\ 
\texttt{p p > a wpm j j } 	 &2 & $2.47 \times 10^{-1}$ & 0.72 & \texttt{p p > t t~ j j } 	 &4 & $6.14 \times 10^{-1}$ & 0.29 \\ 
\texttt{p p > w+ w- wpm} 	 &3 & $1.00 \times 10^{-3}$ & 610.69 & \texttt{p p > t t~ wpm} 	 &2 & $3.58 \times 10^{-1}$ & 1.70 \\ 
\texttt{p p > z w+ w-} 	 &3 & $8.00 \times 10^{-3}$ & 92.39 & \texttt{p p > t t~ z} 	 &2 & $4.58 \times 10^{-1}$ & 1.62 \\ 
\texttt{p p > z z wpm} 	 &3 & $1.00 \times 10^{-2}$ & 85.00 & \texttt{p p > t t~ wpm} 	 &2 & $3.58 \times 10^{-1}$ & 2.37 \\ 
\texttt{p p > z z z } 	 &3 & $1.00 \times 10^{-3}$ & 302.75 & \texttt{p p > t t~ z} 	 &2 & $4.58 \times 10^{-1}$ & 0.66 \\ 
\texttt{p p > a w+ w- } 	 &3 & $1.90 \times 10^{-2}$ & 42.33 & \texttt{p p > t t~ z} 	 &2 & $4.58 \times 10^{-1}$ & 1.76 \\ 
\texttt{p p > a a wpm} 	 &3 & $4.40 \times 10^{-2}$ & 47.24 & \texttt{p p > t t~ a } 	 &2 & $4.44 \times 10^{-1}$ & 4.68 \\ 
\texttt{p p > a z wpm} 	 &3 & $1.00 \times 10^{-3}$ & 1244.49 & \texttt{p p > t t~ wpm} 	 &2 & $3.58 \times 10^{-1}$ & 3.47 \\ 
\texttt{p p > a z z } 	 &3 & $2.00 \times 10^{-2}$ & 17.24 & \texttt{p p > t t~ a } 	 &2 & $4.44 \times 10^{-1}$ & 0.78 \\ 
\texttt{p p > a a z } 	 &3 & $5.60 \times 10^{-2}$ & 8.99 & \texttt{p p > t t~ z} 	 &2 & $4.58 \times 10^{-1}$ & 1.10 \\ 
\texttt{p p > a a a } 	 &3 & $9.80 \times 10^{-2}$ & 17.44 & \texttt{p p > t t~ a } 	 &2 & $4.44 \times 10^{-1}$ & 3.85 \\ 
\texttt{p p > w+ w- wpm j } 	 &3 & $1.50 \times 10^{-1}$ & 2.06 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.48 \\ 
\texttt{p p > z w+ w- j} 	 &3 & $1.56 \times 10^{-1}$ & 1.81 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.44 \\ 
\texttt{p p > z z wmp j } 	 &3 & $1.61 \times 10^{-1}$ & 1.88 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.47 \\ 
\texttt{p p > z z z j } 	 &3 & $1.43 \times 10^{-1}$ & 2.21 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.49 \\ 
\texttt{p p > a w+ w- j} 	 &3 & $1.34 \times 10^{-1}$ & 77781.56 & \texttt{p p > t t~ a j } 	 &3 & $6.05 \times 10^{-1}$ & 17218.16 \\ 
\texttt{p p > a a wpm j } 	 &3 & $1.18 \times 10^{-1}$ & 3.51 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.65 \\ 
\texttt{p p > a z wpm j } 	 &3 & $1.44 \times 10^{-1}$ & 2.30 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.52 \\ 
\texttt{p p > a z z j } 	 &3 & $1.25 \times 10^{-1}$ & 2.96 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.58 \\ 
\texttt{p p > a a z j } 	 &3 & $1.09 \times 10^{-1}$ & 7.57 & \texttt{p p > t t~ z j } 	 &3 & $6.16 \times 10^{-1}$ & 1.34 \\ 
\texttt{p p > a a a j } 	 &3 & $1.43 \times 10^{-1}$ & 6.72 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 1.51 \\ 
\texttt{p p > w+ w- w+ w-} 	 &4 & $3.70 \times 10^{-2}$ & 20.03 & \texttt{p p > t t~ w+ w-} 	 &2 & $6.18 \times 10^{-1}$ & 1.20 \\ 
\texttt{p p > w+ w- wpm z } 	 &4 & $4.40 \times 10^{-2}$ & 19.60 & \texttt{p p > t t~ wpm z} 	 &2 & $5.32 \times 10^{-1}$ & 1.62 \\ 
\texttt{p p > w+ w- wpm a } 	 &4 & $2.50 \times 10^{-2}$ & 36.35 & \texttt{p p > t t~ wpm a } 	 &2 & $5.08 \times 10^{-1}$ & 1.79 \\ 
\texttt{p p > w+ w- z z } 	 &4 & $4.40 \times 10^{-2}$ & 14.68 & \texttt{p p > t t~ z z } 	 &2 & $5.86 \times 10^{-1}$ & 1.10 \\ 
\texttt{p p > w+ w- z a } 	 &4 & $3.00 \times 10^{-2}$ & 25.40 & \texttt{p p > t t~ z a } 	 &2 & $6.02 \times 10^{-1}$ & 1.27 \\ 
\texttt{p p > w+ w- a a } 	 &4 & $6.00 \times 10^{-3}$ & 133.97 & \texttt{p p > t t~ a a } 	 &2 & $5.68 \times 10^{-1}$ & 1.42 \\ 
\texttt{p p > wpm z z z } 	 &4 & $5.10 \times 10^{-2}$ & 21.88 & \texttt{p p > t t~ wpm z} 	 &2 & $5.32 \times 10^{-1}$ & 2.10 \\ 
\texttt{p p > wpm z z a } 	 &4 & $3.60 \times 10^{-2}$ & 43.48 & \texttt{p p > t t~ wpm a } 	 &2 & $5.08 \times 10^{-1}$ & 3.08 \\ 
\texttt{p p > wpm z a a } 	 &4 & $1.70 \times 10^{-2}$ & 110.92 & \texttt{p p > t t~ wpm z} 	 &2 & $5.32 \times 10^{-1}$ & 3.54 \\ 
\texttt{p p > wmp a a a } 	 &4 & $4.00 \times 10^{-3}$ & 618.06 & \texttt{p p > t t~ wpm a } 	 &2 & $5.08 \times 10^{-1}$ & 4.87 \\ 
\texttt{p p > z z z z } 	 &4 & $3.80 \times 10^{-2}$ & 8.46 & \texttt{p p > t t~ z z } 	 &2 & $5.86 \times 10^{-1}$ & 0.55 \\ 
\texttt{p p > z z z a } 	 &4 & $1.90 \times 10^{-2}$ & 16.92 & \texttt{p p > t t~ z a } 	 &2 & $6.02 \times 10^{-1}$ & 0.53 \\ 
\texttt{p p > z z a a } 	 &4 & $1.00 \times 10^{-3}$ & 364.79 & \texttt{p p > t t~ a a } 	 &2 & $5.68 \times 10^{-1}$ & 0.64 \\ 
\texttt{p p > z a a a } 	 &4 & $2.30 \times 10^{-2}$ & 20.97 & \texttt{p p > t t~ z a } 	 &2 & $6.02 \times 10^{-1}$ & 0.80 \\ 
\texttt{p p > a a a a } 	 &4 & $4.70 \times 10^{-2}$ & 24.09 & \texttt{p p > t t~ a a } 	 &2 & $5.68 \times 10^{-1}$ & 1.99 \\ 
\texttt{p p > wpm b b~} 	 &1 & $4.23 \times 10^{-1}$ & 3.92 & \texttt{p p > t t~ b b~} 	 &4 & $4.66 \times 10^{-1}$ & 3.56 \\ 
\texttt{p p > z b b~} 	 &1 & $3.35 \times 10^{-1}$ & 2.31 & \texttt{p p > t t~ b b~} 	 &4 & $4.66 \times 10^{-1}$ & 1.66 \\ 
\texttt{p p > a b b~} 	 &1 & $5.19 \times 10^{-1}$ & 2.72 & \texttt{p p > t t~ b b~} 	 &4 & $4.66 \times 10^{-1}$ & 3.03 \\ 
\texttt{p p > wpm b b~ j} 	 &1 & $4.25 \times 10^{-1}$ & 2.66 & \texttt{p p > t t~ b b~} 	 &4 & $6.21 \times 10^{-1}$ & 1.82 \\ 
\texttt{p p > z b b~ j } 	 &1 & $4.24 \times 10^{-1}$ & 1.78 & \texttt{p p > t t~ b b~} 	 &4 & $6.21 \times 10^{-1}$ & 1.22 \\ 
\texttt{p p > a b b~ j } 	 &1 & $5.12 \times 10^{-1}$ & 1.12 & \texttt{p p > t t~ b b~} 	 &4 & $6.21 \times 10^{-1}$ & 0.93 \\ 
\texttt{p p > t t~ wpm} 	 &1 & $2.39 \times 10^{-1}$ & 2.08 & \texttt{p p > t t~ b b~} 	 &4 & $4.66 \times 10^{-1}$ & 1.07 \\ 
\texttt{p p > t t~ z} 	 &1 & $3.05 \times 10^{-1}$ & 1.45 & \texttt{p p > t t~ b b~} 	 &4 & $4.66 \times 10^{-1}$ & 0.95 \\ 
\texttt{p p > t t~ a } 	 &1 & $2.96 \times 10^{-1}$ & 1.52 & \texttt{p p > t t~ b b~} 	 &4 & $4.66 \times 10^{-1}$ & 0.97 \\ 
\texttt{p p > t t~ wpm j } 	 &1 & $4.09 \times 10^{-1}$ & 1.09 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.70 \\ 
\texttt{p p > t t~ z j } 	 &1 & $4.62 \times 10^{-1}$ & 0.61 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.44 \\ 
\texttt{p p > t t~ a j } 	 &1 & $4.54 \times 10^{-1}$ & 0.67 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.48 \\ 
\texttt{p p > t t~ w+ w-} 	 &2 & $3.09 \times 10^{-1}$ & 1.56 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.76 \\ 
\texttt{p p > t t~ wpm z} 	 &2 & $2.66 \times 10^{-1}$ & 1.77 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.74 \\ 
\texttt{p p > t t~ wpm a } 	 &2 & $2.54 \times 10^{-1}$ & 1.75 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.70 \\ 
\texttt{p p > t t~ z z } 	 &2 & $2.93 \times 10^{-1}$ & 1.24 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.57 \\ 
\texttt{p p > t t~ z a } 	 &2 & $3.01 \times 10^{-1}$ & 1.45 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.68 \\ 
\texttt{p p > t t~ a a } 	 &2 & $2.84 \times 10^{-1}$ & 1.22 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.54 \\ 
\texttt{p p > h} 	 &1 & $3.48 \times 10^{-1}$ & 3.02 & \texttt{p p > t t~} 	 &2 & $1.45 \times 10^{-1}$ & 7.24 \\ 
\texttt{p p > h j } 	 &1 & $3.94 \times 10^{-1}$ & 1.77 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 2.40 \\ 
\texttt{p p > h j j } 	 &1 & $5.91 \times 10^{-1}$ & 1.18 & \texttt{p p > t t~ j } 	 &3 & $4.51 \times 10^{-1}$ & 1.54 \\ 
\texttt{p p > h j j $$ w+ w- z } 	 &4 & $2.00 \times 10^{-2}$ & -2.26 & \texttt{p p > t t~ j } 	 &3 & $5.80 \times 10^{-1}$ & -0.08 \\ 
\texttt{p p > h j j j $$ w+ w- z } 	 &4 & $1.57 \times 10^{-1}$ & 0.61 & \texttt{p p > t t~ j } 	 &3 & $1.05 \times 10^{0}$ & 0.09 \\ 
\texttt{p p > h wpm} 	 &2 & $3.50 \times 10^{-2}$ & 5.24 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 0.63 \\ 
\texttt{p p > h wpm j } 	 &2 & $1.07 \times 10^{-1}$ & 1.91 & \texttt{p p > t t~ j } 	 &3 & $4.51 \times 10^{-1}$ & 0.45 \\ 
\texttt{p p > h wpm j j } 	 &2 & $2.61 \times 10^{-1}$ & 1.18 & \texttt{p p > t t~ j j } 	 &4 & $6.14 \times 10^{-1}$ & 0.50 \\ 
\texttt{p p > h z } 	 &2 & $3.50 \times 10^{-2}$ & 5.30 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 0.64 \\ 
\texttt{p p > h z j } 	 &2 & $1.06 \times 10^{-1}$ & 1.86 & \texttt{p p > t t~ j } 	 &3 & $4.51 \times 10^{-1}$ & 0.44 \\ 
\texttt{p p > h z j j } 	 &2 & $2.62 \times 10^{-1}$ & 0.78 & \texttt{p p > t t~ j j } 	 &4 & $6.14 \times 10^{-1}$ & 0.33 \\ 
\texttt{p p > h w+ w-} 	 &3 & $1.00 \times 10^{-3}$ & 284.51 & \texttt{p p > h t t~} 	 &2 & $4.50 \times 10^{-1}$ & 0.63 \\ 
\texttt{p p > h wpm a} 	 &3 & $7.00 \times 10^{-3}$ & 44.78 & \texttt{p p > h t t~} 	 &2 & $4.50 \times 10^{-1}$ & 0.70 \\ 
\texttt{p p > h z wpm} 	 &3 & $1.10 \times 10^{-2}$ & 36.99 & \texttt{p p > h t t~} 	 &2 & $4.50 \times 10^{-1}$ & 0.90 \\ 
\texttt{p p > h z z } 	 &3 & $1.00 \times 10^{-3}$ & 215.31 & \texttt{p p > h t t~} 	 &2 & $4.50 \times 10^{-1}$ & 0.48 \\ 
\texttt{p p > h t t~} 	 &1 & $3.00 \times 10^{-1}$ & 0.96 & \texttt{p p > t t~ t t~} 	 &4 & $4.79 \times 10^{-1}$ & 0.60 \\ 
\texttt{p p > h tt j} 	 &1 & $2.40 \times 10^{-2}$ & 11.19 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.42 \\ 
\texttt{p p > h b b~} 	 &1 & $2.81 \times 10^{-1}$ & 0.79 & \texttt{p p > t t~ t t~} 	 &4 & $4.79 \times 10^{-1}$ & 0.47 \\ 
\texttt{p p > h t t~ j } 	 &1 & $4.56 \times 10^{-1}$ & 0.47 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.33 \\ 
\texttt{p p > h b b~ j } 	 &1 & $4.56 \times 10^{-1}$ & 0.49 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.35 \\ 
\texttt{p p > h h } 	 &2 & $2.95 \times 10^{-1}$ & 1.90 & \texttt{p p > t t~} 	 &2 & $2.90 \times 10^{-1}$ & 1.93 \\ 
\texttt{p p > h h j j $$ w+ w- z} 	 &5 & $7.20 \times 10^{-2}$ & 0.68 & \texttt{p p > t t~ t t~} 	 &4 & $1.12 \times 10^{0}$ & 0.04 \\ 
\texttt{p p > h h wpm} 	 &3 & $9.00 \times 10^{-3}$ & 18.09 & \texttt{p p > t t~ wpm} 	 &2 & $3.58 \times 10^{-1}$ & 0.45 \\ 
\texttt{p p > h h wpm j} 	 &3 & $1.42 \times 10^{-1}$ & 1.10 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.24 \\ 
\texttt{p p > h h wpm a} 	 &4 & $3.00 \times 10^{-2}$ & 6.84 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.32 \\ 
\texttt{p p > h h z } 	 &3 & $9.00 \times 10^{-3}$ & 17.70 & \texttt{p p > t t~ t t~} 	 &4 & $4.79 \times 10^{-1}$ & 0.33 \\ 
\texttt{p p > h h z j } 	 &3 & $1.41 \times 10^{-1}$ & 1.06 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.23 \\ 
\texttt{p p > h h z a } 	 &4 & $2.40 \times 10^{-2}$ & 5.95 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.22 \\ 
\texttt{p p > h h z z } 	 &4 & $3.90 \times 10^{-2}$ & 4.88 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.30 \\ 
\texttt{p p > h h z wpm} 	 &4 & $4.80 \times 10^{-2}$ & 6.68 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.50 \\ 
\texttt{p p > h h w+ w-} 	 &4 & $3.50 \times 10^{-2}$ & 6.65 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.36 \\ 
\texttt{p p > h h t t~} 	 &2 & $3.02 \times 10^{-1}$ & 0.26 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.13 \\ 
\texttt{p p > h h tt j} 	 &2 & $1.00 \times 10^{-3}$ & 326.09 & \texttt{p p > t t~ t t~} 	 &4 & $7.97 \times 10^{-1}$ & 0.41 \\ 
\texttt{p p > h h b b~} 	 &2 & $3.43 \times 10^{-1}$ & 1.10 & \texttt{p p > t t~ t t~} 	 &4 & $6.38 \times 10^{-1}$ & 0.59 \\ 

